Learning from Peers at the Wireless Edge

The last mile connection is dominated by wireless links where heterogeneous nodes share the limited and already crowded electromagnetic spectrum. Current contention based decentralized wireless access system is reactive in nature to mitigate the interference. In this paper, we propose to use neural networks to learn and predict spectrum availability in a collaborative manner such that its availability can be predicted with a high accuracy to maximize wireless access and minimize interference between simultaneous links. Edge nodes have a wide range of sensing and computation capabilities, while often using different operator networks, who might be reluctant to share their models. Hence, we introduce a peer to peer Federated Learning model, where a local model is trained based on the sensing results of each node and shared among its peers to create a global model. The need for a base station or access point to act as centralized parameter server is replaced by empowering the edge nodes as aggregators of the local models and minimizing the communication overhead for model transmission. We generate wireless channel access data, which is used to train the local models. Simulation results for both local and global models show over 95% accuracy in predicting channel opportunities in various network topology.

==> hidding_prob.tex <==
\section{Solving hiding terminal problem}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/hiding.jpg}
    \caption{Network Topology.}
    \label{fig:net}
    \vspace{-15pt}
\end{figure}


Each node $N_{i}$ generates its local parameter $\theta_{i}$ based on the collected sensing data. The local model parameters are shared via a broadcast signal. However, the sensing data does not capture all the dynamics of the network. Thus For each node $N_{i}$ constructs a global model. The global model parameters is a function of its local parameters as well as the local parameters of the surrounding nodes. Consequently,  the global model parameters can be expressed as: 
\begin{equation}
    \Theta_{i}=  \frac{1}{M}\sum_{l=1}^{M} \theta_{l}
    \label{eq:glob}
\end{equation}
where $\theta_{l}$ is the local model parameters of $N_{i}$ or the surrounding nodes. As shown in (\ref{eq:glob}), the global model is adjusted by averaging its local model with the surrounding nodes. Consequently, the hiding terminal problem is solved because the global model is a function of all the surrounding nodes including the hidden terminal. On the other hand, sharing the local model parameters enable the network to solve the redundancy of the model parameters, since each local model depends on its sensed data.
















